Federated Ensemble-Directed Offline Reinforcement Learning

We consider the problem of federated offline reinforcement learning (RL), a scenario under which distributed learning agents must collaboratively learn a high-quality control policy only using small pre-collected datasets generated according to different unknown behavior policies. Na\"{i}vely combining a standard offline RL approach with a standard federated learning approach to solve this problem can lead to poorly performing policies. In response, we develop the Federated Ensemble-Directed Offline Reinforcement Learning Algorithm (FEDORA), which distills the collective wisdom of the clients using an ensemble learning approach. We develop the FEDORA codebase to utilize distributed compute resources on a federated learning platform. We show that FEDORA significantly outperforms other approaches, including offline RL over the combined data pool, in various complex continuous control environments and real-world datasets. Finally, we demonstrate the performance of FEDORA in the real-world on a mobile robot. We provide our code and a video of our experiments at \url{https://github.com/DesikRengarajan/FEDORA}.

==> Sections/Introduction.tex <==
\section{Introduction}

 Federated learning is an approach wherein clients learn collaboratively by sharing their locally trained models (not their data) with a federating agent, which periodically combines their models and returns the federated model to the clients for further refinement \citep{kairouz2021advances, wang2021field}.  Federated learning has seen much success in supervised learning applications due to its ability to generate well-trained models using small amounts of data at each client while preserving privacy and reducing the usage of communication resources. Recently, there is a growing interest in employing federated learning for \emph{online} RL problems where  each client collects data online by following its own Markovian trajectory, while simultaneously updating the model parameters \citep{khodadadian2022federated, nadiger2019federated, qi2021federated}. However, such an online learning approach requires  sequential interactions with the environment, which  may not be feasible in many real-world applications. Instead, each clients may have pre-collected operational data generated according to a client-specific  behavior policy. The \emph{federated offline reinforcement learning} problem is to   learn the optimal policy using these heterogeneous offline data sets distributed across the clients and collected  by different unknown behavior policies,   without sharing the data explicitly.  
 

The framework of offline reinforcement learning \citep{offtutorial} offers a way to learn  the policy only using the offline data collected according a behavior policy, without any environment interactions. However, naively combining an off-the-shelf offline RL algorithm such as TD3-BC \citep{fujimoto2021minimalist} with an off-the-shelf  federated supervised learning approach such as FedAvg \citep{mcmahan2017communication} will lead to a poorly performing  policy, as we show later (see Fig.~\ref{fig:why1}-\ref{fig:sim_mujoco}). Federated offline RL is significantly more challenging than its supervised learning counterpart and the centralized offline RL because of the following reasons. (i) \emph{Ensemble heterogeneity:} Client datasets are collected according to different behavior policies with different performance levels.  It is vital to capture the collective insight of these policies rather than merely average them. (ii) \emph{Pessimistic value computation:} Offline RL algorithms employ  a notion of pessimism with respect to the offline data for minimizing the distribution shift. However, in a federated setting, it is important capture the information from data of other clients.  (iii) \emph{Data heterogeneity:} Client drift caused by multiple local updates on heterogeneous data may lead to biased and poor performing federated models. 



In this work, we propose the federated ensemble-directed offline RL algorithm (FEDORA), which can overcome these challenges to obtain high-quality control policies collaboratively. Our proposed approach recognizes that individual client policies are of varying levels of expertise
and refines the federated policy based on the relative merits of each client policy in an ensemble learning manner. The algorithm combines the insight across critics similarly and ensures optimism across the federated and local critics, thereby setting ambitious targets for training. FEDORA addresses the issue of data heterogeneity by regularizing the client policies with respect to both the federated policy and the local dataset. Finally, FEDORA prunes the influence of irrelevant data by gradually decaying the reliance on a dataset based on the quality of the policy it can generate.

Federated offline RL has not been well studied in the literature, and to the best of our knowledge, no other work presents an approach that addresses the general problem. The primary contribution of this work is to systematically identify the  fundamental challenges of this problem and design methods that explicitly tackle each of them. 
%The idea of learning over an ensemble of policies of different qualities to leverage their collective insight is unique to our method.  

We develop a framework for implementing  FEDORA  on a single system and over distributed compute resources. We evaluate FEDORA on standard MuJoCo environments and real world datasets and show that it outperforms several other approaches, including pooling all the data and performing offline RL centrally.  We also demonstrate FEDORA's excellent performance via real world experiments on a TurtleBot robot \citep{amsters2019turtlebot}.  We provide the code for our implementation and the  videos of the robot experiments in the supplementary material.  %\url{https://github.com/DesikRengarajan/FEDORA}. 




==> Sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{appdx:limitations}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appendix \ref{apdx:setup} and code \url{https://github.com/DesikRengarajan/FEDORA}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See code \url{https://github.com/DesikRengarajan/FEDORA}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See section \ref{sec:exp1}, Appendix \ref{apdx:setup}, and code in \url{https://github.com/DesikRengarajan/FEDORA}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See section \ref{sec:exp1}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appendix \ref{apdx:setup}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See section \ref{sec:impact}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code at \url{https://github.com/DesikRengarajan/FEDORA} and Appendix \ref{apdx:setup}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See code at \url{https://github.com/DesikRengarajan/FEDORA}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> Sections/fedora.tex <==


\section{Federated Offline Reinforcement Learning}\label{sec:FORL}

In real-world offline RL applications, the data is typically obtained from the operational policies of multiple agents (clients) with different levels of expertise. Often, clients prefer to keep their operational data local without sharing it with others. A federated offline RL algorithm aims to learn the optimal policy for the underlying RL problem using the available offline data without the clients sharing their data with one another or the server. We denote the set of clients as $\mathcal{N}$. Each client $i \in  \mathcal{N}$ has the offline dataset $\mathcal{D}_i = \{(s_{j}, a_{j}, r_{j}, s'_{j})^{m_{i}}_{j=1}\}$ generated according to a behavior policy $\pi^{b}_{i}$.   We assume that the underlying MDP model $P$ and reward function $R(\cdot, \cdot)$ are identical for all the clients, and the statistical differences between the offline datasets $\mathcal{D}_i$ are only due to the difference in behavior policies $\pi^{b}_{i}$ used for collecting the data. 

In a standard federated learning algorithm such as FedAvg, each client performs multiple parameter updates before sending its parameters to the server. {It is known that performing multiple local updates in federated learning can reduce the communication cost significantly without compromising on the optimality of the converged solution  \citep{kairouz2021advances, wang2021field}}. In federated offline RL, since each client has to perform multiple steps of policy evaluation and policy update using its local offline data $\mathcal{D}_{i}$,  it is reasonable to consider a client objective function that is consistent with a standard offline RL algorithm objective. We choose the objective function used in the TD3-BC algorithm \citep{fujimoto2021minimalist}, i.e., $U_{\mathcal{D}_i}$  given in Eq.~\eqref{eq:td3_bc1}, as the client objective function. Our choice is motivated by the simplicity of the TD3-BC objective function and its empirical success in a variety of environments. Similar to the standard federated learning objective given in Eq.~\eqref{eq:fed_objective}, we can now define the federated offline RL objective as
\begin{align}
\label{eq:fedRL_obj}
    U(\pi_{\text{fed}}) = \sum_{i = 1}^{|\mathcal{N}|} w_i U_{\mathcal{D}_i}(\pi_{\text{fed}}),
\end{align}
where $w_i$ are weights to be determined. 






One approach to leveraging experiences across users without sharing data would be to combine existing federated learning techniques with offline RL algorithms. \emph{Is such a na\"{\i}ve federation strategy sufficient to learn an excellent federated policy collaboratively? Furthermore, is federation even necessary?} In this section, we aim to understand the challenges of federated offline RL with the goal of designing an algorithmic framework to address these challenges. 


We start with an example illustrating the issues in designing a federated offline RL algorithm. We consider the Hopper environment from MuJoCo \citep{todorov2012mujoco}, with $|\mathcal{N}| = 10$, $|\mathcal{D}_{i}| = 5000$, and we use the data from the D4RL dataset \citep{fu2020d4rl}. However, instead of using the data generated by the same policy for all clients, we consider the setting where five clients use the data from the hopper-expert-v2 dataset (which was generated using a completely trained (expert) SAC policy) and five clients use the data from the hopper-medium-v2 dataset (which was generated using a partially trained (medium) policy achieving only a third of the expert performance). The clients and the server are unaware of the quality (expert or medium) of the data. Fig.~\ref{fig:why1} shows the performance comparison of multiple algorithms, where the mean and the standard deviation are calculated over $4$ seeds.

\begin{wrapfigure}[12]{r}{0.35\linewidth}
    \centering
    \vspace{-\intextsep}
    \includegraphics[width=1\linewidth]{Figures/Introduction/plot_why.pdf}
    \caption{Performance comparison of federated and centralized offline RL algorithms.}
    \label{fig:why1}
\end{wrapfigure}


\textbf{Combining All Data (Centralized):}  Combining data and learning centrally is the ideal scenario in supervised learning. However, as seen in Fig.~\ref{fig:why1}, performing centralized training over combined data generated using different behavior policies in offline RL can be detrimental. Sharing data can exacerbate the distributional shift between the learned policy and the individual datasets, leading to 
 poor performance. Such performance deterioration due to combining data from behavior policies with different expertise levels has been observed in the offline RL literature \citep{yu2021conservative,fujimoto2021minimalist,cql}.
    


\textbf{Individual Offline RL:} Here, agents apply offline RL to their own datasets without collaborating with others. In Fig.~\ref{fig:why1}, we observe that clients with either expert or medium data do not learn well and exhibit a large standard deviation. This observation may be attributed to no client having sufficient data to learn a good policy. 



\textbf{Na\"{\i}ve Federated Offline RL:} A simple federation approach is to use the offline RL objective as the local objective and apply FedAvg (Eq.~\eqref{eq:fed_avg}). However, offline RL algorithms typically comprise two components -- an actor and a critic. It is unclear a priori which components should be federated, so we conduct experiments where we federate only the actor (Fed-A) or both the actor and the critic (Fed-AC). Surprisingly, these na\"{\i}ve strategies result in federated policies that perform worse than individual offline RL, as witnessed in Fig.~\ref{fig:why1}.


\subsection{Issues with Federated Offline RL}

Our example illustrates several fundamental issues that must be addressed while designing viable federated offline RL algorithms, including:

\textbf{1. Ensemble Heterogeneity:}  Performing offline RL over heterogeneous data yields a set of policies of different qualities. 
It is crucial to leverage the information contained in these varied policies rather than simply averaging them. However, federation after a single-step local gradient at each client using weights in the manner of FedAvg, $w_i = |\mathcal{D}_i|/|\sum_{i=1}^{|\mathcal{N}|}|\mathcal{D}_i|$, is equivalent to solving the offline RL problem using the combined dataset of all clients \citep{wang2021field}. This approach leads to poor performance due to the resulting distribution shift, as shown in Fig.~\ref{fig:why1}. \emph{How should we optimally federate the ensemble of policies learned by the clients?}

\textbf{2. Pessimistic Value Computation:}  Most offline RL algorithms involve a pessimistic term with respect to the offline data for minimizing the distribution shift. Training a client critic using only the local data with this pessimistic term could make it pessimistic towards actions poorly represented in its dataset but well represented in other clients' data.  \emph{How do we effectively utilize the federated critic along with the locally computed critic to set ambitious targets for offline RL at each client?}      

 \textbf{3. Data Heterogeneity:} Federated learning calls for performing multiple local gradient steps at each client before federation to enhance communication efficiency. However, numerous epochs would bias a client's local model to its dataset. This client drift effect is well known in federated (supervised) learning and could lead to policies that are not globally optimal. In turn, this could cause the federated policy's performance to be worse than training locally using only the client's data, as seen in Fig.~\ref{fig:why1}. \emph{How should we regularize local policies to prevent this?}



\section{FEDORA Design Approach}\label{sec:FEDORA}

We desire to develop a Federated Ensemble-Directed Offline RL Algorithm (FEDORA) that addresses the issues outlined in Section \ref{sec:FORL} in a systematic manner. Three fundamental requirements drive our approach. First, the clients jointly possess an ensemble of local policies of different levels of quality, and the server must leverage the collective knowledge embedded in this ensemble during federation. Second, the quality of these policies must be assessed using an ensemble of critics that depend on local data for policy evaluation. Finally, after each round of federation, clients must update their local policies via offline RL utilizing both their local data and the received federated policy.

We begin by considering the objective of ensemble learning at federation. We define $p_i$  as a measure of the relative priority of the local policy obtained from client $i.$  Then, the weights $w_{i}$ in  the federated offline RL objective (Eq.~\eqref{eq:fedRL_obj}) can be defined as 
\begin{align}
\label{eq:fed-rl-weights}
    {w}_i &= \frac{ p_i|\mathcal{D}_i|}{|\mathcal{D}|}, \quad |\mathcal{D}| = \sum_{i = 1}^{|\mathcal{N}|} p_i|\mathcal{D}_i|.
\end{align}
Based on this objective, we now design FEDORA accounting for each of the three requirements indicated above. In what follows, we will denote the round of federation using a super-script $t$ and local update step within a round of federation by the super-script $k$. More precisely, $\pi^{(t,k)}_{i}$ denotes the policy of client $i$ in round $t$ of federation after $k$ local policy updates.  Since all clients initialize their local policies to the federated policy at the beginning of each round of federation, $\pi^{(t,0)}_{i} = \pi_{\text{fed}}^{t}$ for each client $i$. We also denote $\pi^{t}_{i} = \pi^{(t,K)}_{i}$, where $K$ is the maximum number of local updates. Since all clients initialize their local critics to the federated critic, we can similarly define $Q^{(t,k)}_i$,   $Q^{(t,0)}_i = Q^t_{\text{fed}}$, and $Q^t_i = Q^{(t,K)}_i$ for the local  critic. 

% We desire to develop a Federated Ensemble-Directed Offline RL Algorithm (FEDORA) that addresses the issues outlined in Section \ref{sec:FORL} in a systematic manner. Three fundamental requirements drive our approach. First, the clients jointly possess an ensemble of local policies of different levels of quality, and the server must leverage the collective knowledge embedded in this ensemble during federation. Second, the quality of these policies must be assessed using an ensemble of critics that depend on local data for policy evaluation. Finally, after each round of federation, clients must update their local policies via offline RL utilizing both their local data and the received federated policy

% We  design FEDORA accounting for each of the three requirements indicated above. In what follows, we will denote the round of federation using a super-script $t$ and local update step within a round of federation by the super-script $k$. More precisely, $\pi^{(t,k)}_{i}$ denotes the policy of client $i$ in round $t$ of federation after $k$ local policy updates.  Since all clients initialize their local policies to the federated policy at the beginning of each round of federation, $\pi^{(t,0)}_{i} = \pi_{\text{fed}}^{t}$ for each client $i$. We also denote $\pi^{t}_{i} = \pi^{(t,K)}_{i}$, where $K$ is the maximum number of local updates. Since all clients initialize their local critics to the federated critic, we can similarly define $Q^{(t,k)}_i$,   $Q^{(t,0)}_i = Q^t_{\text{fed}}$, and $Q^t_i = Q^{(t,K)}_i$ for the local  critic.

 \subsection{Ensemble-Directed Learning over Client Policies}


As seen in Fig.~\ref{fig:why1}, na\"{\i}vely federating offline RL results in policies that perform worse than learning on aggregated data, which is itself sub-optimal (and not feasible in a federated setting). Furthermore, simply averaging over the clients' policies without considering their qualities implies that low-quality policies will have the same influence on the federated policy as high-quality ones. Such an averaging technique could lead to a scenario where the federated policy's performance is worse than training locally using only a client's data. We desire an ensemble learning approach that continually refines the federated policy based on the relative merits of the client policies over multiple rounds of federation. 

The figure of merit for a given client $i$'s local policy at round $t$, $\pi_i^{t}$, is its infinite horizon discounted reward $J\left(\pi_{i}^{t}\right)$. However, while obtaining an unbiased estimate of the performance of a policy in the online RL setting is straightforward, it is hard to do so in offline RL since we do not have access to the environment for executing the policy and evaluating its performance. Therefore, we use the offline data to get a proxy estimate $J_i^t$ for the quality of the final local policy $\pi_i^{t}$ as $ J^t_i  = \mathbb{E}_{s \sim \mathcal{D}_i}\left[ Q^{t}_i(s,\pi^{t}_i(s)) \right]  \label{eq:pol_val},$ where $Q_i^{t}$ is the local critic function at round $t$ after $K$ local updates (computation of $Q_i^{t}$ and $\pi^{t}_{i}$ are described later). We then  compute the relative priority $p_i^t$ (Eq. \eqref{eq:p_FedAvg}) of client $i$ at round $t$ using a soft-max function  
%as 
% \begin{align}
%     p_i^t &= \frac{e^{\beta J^t_i}}{\sum_{i = 1}^{|\mathcal{N}|} e^{\beta J^t_i}}, 
% \end{align}
where $\beta$ is a tunable temperature parameter.  The weights $w_{i}$s in the federated offline RL objective (Eq.~\eqref{eq:fedRL_obj}) can now be defined as in Eq.~\eqref{eq:fed-rl-weights} using the relative priority $p_i^t$s. Finally, the server updates the federated policy as 
\begin{align}
   p_i^t = \frac{e^{\beta J^t_i}}{\sum_{i = 1}^{|\mathcal{N}|} e^{\beta J^t_i}}, \quad
    \pi_{\text{fed}}^{t+1} = \sum_{i = 1}^{|\mathcal{N}|} w^t_i \pi_i^{t}. \label{eq:p_FedAvg}
\end{align}

% Solving the federated offline reinforcement learning (RL) problem in equation \eqref{eq:fedRL_obj} using the weights chosen by FedAvg is equivalent to solving the offline RL problem using the combined dataset of all clients. This can lead to poor performance because combining data can exacerbate the distribution shift problem that affects offline RL algorithms. Offline RL algorithms typically address the distribution shift problem by implicitly or explicitly constraining the learned policy to stay close to the behavior policy that generated the data. However, if low-quality data is added to the training data, this constraint will cause the learned policy to change, resulting in a lower-quality learned policy. 
 
%  Additionally, averaging the clients' policies without considering their quality means that low-quality policies will have the same impact on the federated policy as high-quality ones. This could lead to a situation where the federated policy's performance is worse than training locally using only a single client's data. We want an ensemble learning approach that continuously improves the federated policy based on the relative merits of the client policies over multiple rounds of federation. 

% We aim to over come this issue by combining data of clients based on their expertise or Q-values. While this process is straightforward in the data sharing regime \citep{yu2021conservative}, its not clear on how to achieve this in the federated setting. Our goal is to modify the weighing scheme, such that we are able to bias the federated model towards clients that possess data that can lead to good federated policies. To achieve this, we would like to maximize the the objective in Eq. \eqref{eq:fedRL_obj} over the weights $w_i$ as well. To prevent the weights from collapsing over a few clients, and to encourage useful data sharing amongst clients, we add an entropy regularization with temperature parameter $\beta$ over the weights resulting in the following objective.  
% \begin{align}
% \label{eq:fedRL_entropy}
%     U(\pi_{\text{fed}}) = \sum_{i = 1}^{|\mathcal{N}|} w_i U_{\mathcal{D}_i}(\pi_{\text{fed}}) - \frac{1}{\beta} \sum_{i = 1}^{|\mathcal{N}|} w_i \log w_i.
% \end{align}

% \begin{lemma}
% The maximum of Eq. \ref{eq:fedRL_entropy} is reached when weights $w_i = \frac{e^{\beta  U_{\mathcal{D}_i}(\pi_{\text{fed}})}}{\sum_{i = 1}^{|\mathcal{N}|} e^{\beta  U_{\mathcal{D}_i}(\pi_{\text{fed}})}}$. 
% % \begin{proof}
% % Take Lagrangian and solve dual.
% % \end{proof}
% \end{lemma}

%  This calls for averaging the weights after the completion of local training, which in the federated learning setting can be detrimental, as the local models can deviate farther from the federated model \citep{wang2021field,karimireddy2020scaffold}. To prevent this, we federate after $K$ local epochs. In practice we compute the weight $w^t_i$ of client $i$ in round $t$ by accounting for the size of the local dataset, and using the estimate of the performance of the final local policy $ J^t_i  = \mathbb{E}_{s \sim \mathcal{D}_i}\left[ Q^{t}_i(s,\pi^{t}_i(s)) \right],$ where $Q_i^{t}$ is the local critic function at round $t$ after $K$ local updates (computation of $Q_i^{t}$ and $\pi^{t}_{i}$ are described later).
% \begin{align}
%    w_i^t = \frac{e^{\beta J^t_i} |\mathcal{D}_i| }{\sum_{i = 1}^{|\mathcal{N}|} e^{\beta J^t_i} |\mathcal{D}_i|}, \quad
%     \pi_{\text{fed}}^{t+1} = \sum_{i = 1}^{|\mathcal{N}|} w^t_i \pi_i^{t}.  \label{eq:p_FedAvg}
% \end{align}

% We thus have an ensemble learning approach, where we continually refine the federated policy based on the relative merits of the client policies over multiple rounds of federation.  

 


\subsection{Federated Optimism for Critic Training}


The critic in our algorithm plays two major roles. First, offline RL for policy updates at each client requires policy evaluation using local data. Second, policy evaluation by the critic determines the priority $p_i^t$ of the local policy at client $i$ for ensemble learning during each round $t$ of federation. We desire a local critic at each client that can utilize the knowledge from the ensemble of critics across all clients while also being tuned to the local data used for policy evaluation.

% A critic based on offline data suffers from extrapolation errors as state-actions pairs not seen in the local data  will be erroneously estimated.  Such errors have a large impact on actor-critic style policy updates after each federation round, since the federated policy is derived from the ensemble of local policies and so it may  take actions that are not seen in the local dataset of each individual client. This problem is exacerbated when the local policy at the beginning of each round of federation is initialized to the federated policy.  We introduce the notion of \textit{federated optimism} to train local critics, wherein critics leverage the wisdom of the crowd and are encouraged to be optimistic. We achieve this federated optimism via two steps. 

A critic based on offline data suffers from extrapolation errors as state-actions pairs not seen in the local dataset will be erroneously estimated, greatly impacting actor-critic style policy updates in federated offline RL. Since the federated policy is derived from the set of local policies, it may take actions not seen in any client's local dataset. This problem is exacerbated when the local policy at the beginning of each communication round is initialized to the federated policy. We introduce the notion of \textit{federated optimism} to train local critics, wherein critics leverage the wisdom of the crowd and are encouraged to be optimistic. We achieve this federated optimism via two steps. 

First, we use an ensemble-directed federation of the critics, where the local critic of client $i$ at round $t$ is weighed according to its merit to compute the federated critic as
\begin{align}
    Q_{\text{fed}}^{t+1} = \sum_{i = 1}^{|\mathcal{N}|} w^t_i Q_i^{t} \label{eq:critic_fed}.
\end{align} 
Such a priority-weighted averaging ensures that the critics from clients with good policies significantly influence the federated critic.


Second, for the local critic update, we  choose the target value as  the maximum value between the local critic and the federated critic, given by $\tilde{Q}_i^{(t,k)}(s,a) = \max\left(Q_i^{(t,k)}(s,a),Q_{\text{fed}}^t(s,a)\right),$
% \begin{align}\label{eq:target}
%     \tilde{Q}_i^{(t,k)}(s,a) = \max\left(Q_i^{(t,k)}(s,a),Q_{\text{fed}}^t(s,a)\right),  
% \end{align}
where  $\tilde{Q}_i^{(t,k)}(s,a)$ is the target value of state $s$ and action $a$ at the $t^\text{th}$ round of federation after $k$ local critic updates. This ensures that the local critic has an optimistic (but likely feasible) target seen by the system. Using this optimistic target in the Bellman error, we update the local critic as
\begin{align}
\label{eq:critic_update}
    Q^{(t,k+1)}_{i} = \argmin_{Q} ~ \mathbb{E}_{(s,a,r,s') \sim \mathcal{D}_i} [ ( r &+ \gamma \tilde{Q}_i^{(t,k)}(s',a')- Q(s,a))^{2}], 
\end{align}
where  $a' = \pi^{(t,k)}_{i}$. 
In practice, instead of solving the entire optimization problem described above, we obtain $ Q^{(t,k+1)}_{i}$ after a single gradient update w.r.t. the objective function. 


\subsection{Proximal Policy Update for Heterogeneous Data}
While essential in order to set ambitious estimates, an optimistic critic might erroneously estimate the value of $\tilde{Q}_i^{(t,k)}$. Therefore, regularizing the local policy update w.r.t. both the local data and the federated policy is crucial. For regularization w.r.t. to the local offline data, we use the same method as in the TD3-BC algorithm and define the local loss function $\mathcal{L}_{\text{local}}(\pi) = \mathbb{E}_{(s,a) \sim \mathcal{D}_i}[ -Q_i^{(t,k)}(s,\pi(s)) + (\pi(s) - a)^2]$. We then define the actor loss $\mathcal{L}_{\text{actor}}$ in Eq. \eqref{eq:actor_loss_update}, where the second term is a regularization w.r.t. to the federated policy. The local policy is updated using $\mathcal{L}_{\text{actor}}$, and similar to the local critic update, we perform only one gradient update w.r.t. $\mathcal{L}_{\text{actor}}$ to obtain $\pi^{t,k+1}_{i}$, instead of solving the complete optimization problem above.
% % \begin{align}
% %     \mathcal{L}_{\text{local}}(\pi) = \mathbb{E}_{(s,a) \sim \mathcal{D}_i}[ -Q_i^{(t,k)}(s,\pi(s)) + (\pi(s) - a)^2] \label{eq:local_loss}.
% % \end{align}
% We then define the actor loss $\mathcal{L}_{\text{actor}}$ as
\begin{align}
\label{eq:actor_loss_update} 
    \mathcal{L}_{\text{actor}}(\pi) =  \mathcal{L}_{\text{local}}(\pi) + \mathbb{E}_{(s,a) \sim \mathcal{D}_i}[  (\pi(s) - \pi^t_{\text{fed}}(s))^2], \quad \pi^{t,k+1}_{i} = \argmin_{\pi} ~ \mathcal{L}_{\text{actor}}(\pi).
\end{align}
% where the second term is a regularization w.r.t. to the federated policy. The local policy is updated using $\mathcal{L}_{\text{actor}}$ as
% \begin{align}\label{eq:actor_update}
%     \pi^{t,k+1}_{i} = \argmin_{\pi} ~ \mathcal{L}_{\text{actor}}(\pi). 
% \end{align}
% Similar to the local critic update, we perform only one gradient update w.r.t. $\mathcal{L}_{\text{actor}}$ to obtain $\pi^{t,k+1}_{i}$, instead of solving the complete optimization problem above.






\subsection{Decaying the Influence of Local Data}\label{sec:decay}


FEDORA uses a combination of local data loss and a proximal term for its policy update Eq. \eqref{eq:actor_loss_update}. However, the local data loss might hamper the updated policy's performance since the local dataset may be generated according to a non-expert behavior policy. Hence, a client must decay the influence of its local data if it is reducing the performance of the updated policy by lowering the influence of $\mathcal{L}_{\text{local}}$ in $\mathcal{L}_{\text{actor}}$. To do so, we first evaluate the performance of the federated policy using the federated critic and local data at round $t$. For this evaluation, we use the proxy estimate $J_i^{\text{fed},t} = \mathbb{E}_{s \sim \mathcal{D}_i} \left[ Q_\text{fed}^t (s,\pi^t_\text{fed}(s))\right]$. We compare this value with the performance of the updated policy, $J_i^t$, which is obtained using the updated critic. This difference provides us with an estimate of the improvement the local data provides. We decay the influence of $\mathcal{L}_{\text{local}}$ by a factor $\delta$ if $J_i^{\text{fed},t} \geq J^t_i$. We summarize FEDORA in Algorithm \ref{algo:client} and \ref{algo:server}. 


\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{Outline of Client $i$'s Algorithm}
\begin{algorithmic}[1]
\FUNCTION{train\_client($\pi^t_{\text{fed}}$, $Q^t_{\text{fed}}$)}
\STATE $\pi_i^{(t,0)} = \pi^t_{\text{fed}}, \quad Q^{(t,0)}_i = Q^t_{\text{fed}}$
\FOR{$1 \leq k < K $}
\STATE Update Critic by one gradient step w.r.t. Eq.~\eqref{eq:critic_update}
\STATE Update Actor  by one gradient step w.r.t. Eq.~\eqref{eq:actor_loss_update} 
\ENDFOR
\STATE Decay $\mathcal{L}_{\text{local}}$ by $\delta$ if $J_i^{\text{fed},t} \geq J^t_i$
\ENDFUNCTION
\end{algorithmic}
\label{algo:client}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\caption{Outline of Server Algorithm}
\begin{algorithmic}[1]
\STATE Initialize $\pi^1_{\text{fed}},Q^1_{\text{fed}}$
\FOR{$t \in 1 \dots$}
\STATE Send $\pi^t_{\text{fed}}$ and $Q^t_{\text{fed}}$ to $i \in \mathcal{N}$
\STATE Sample $\mathcal{N}_t \subset \mathcal{N}$
\FOR{ $i \in \mathcal{N}_t$}
\STATE $i$.train\_client $(\pi^t_{\text{fed}},Q^t_{\text{fed}})$
\ENDFOR
\STATE Compute $\pi_{\text{fed}}^{t+1}$ and $Q_{\text{fed}}^{t+1}$ for clients in $\mathcal{N}_t$ using Eq. ~\eqref{eq:p_FedAvg} and ~\eqref{eq:critic_fed} respectively. 
\ENDFOR
\end{algorithmic}
\label{algo:server}
\end{algorithm}
\end{minipage}


